OpenMP Advisor

With the increasing diversity of heterogeneous architecture in the HPC industry, porting a legacy application to run on different architectures is a tough challenge. In this paper, we present OpenMP Advisor, a first of its kind compiler tool that enables code offloading to a GPU with OpenMP using Machine Learning. Although the tool is currently limited to GPUs, it can be extended to support other OpenMP-capable devices. The tool has two modes: Training mode and Prediction mode. The training mode must be executed on the target hardware. It takes benchmark codes as input, generates and executes every variant of the code that could possibly run on the target device, and then collects data from all of the executed codes to train an ML-based cost model for use in prediction mode. However, in prediction mode the tool does not need any interaction with the target device. It accepts a C code as input and returns the best code variant that can be used to offload the code to the specified device. The tool can determine the kernels that are best suited for offloading by predicting their runtime using a machine learning-based cost model. The main objective behind this tool is to maintain the portability aspect of OpenMP. Using our Advisor, we were able to generate code of multiple applications for seven different architectures, and correctly predict the top ten best variants for each application on every architecture. Preliminary findings indicate that this tool can assist compiler developers and HPC application researchers in porting their legacy HPC codes to the upcoming heterogeneous computing environment.

==> code/code.tex <==
\renewcommand{\lstlistingname}{Code}
\begin{figure*}[!htb]
\centering
\vspace{-2em}\noindent
\begin{minipage}{.39\textwidth}
\begin{lstlisting}[caption=Two kernels using same data,frame=tlrb]{Name}
/*Kernel 1 using array A*/
for(...) { ... }
/*Kernel 1 End*/
<@\color{mauve}{/*Serial Code Start}@>
<@\color{mauve}{...}@> // with no dependency on any kernel
<@\color{mauve}{Serial Code End*/}@>
/*Kernel 2  using array A*/
for(...) { ... }
/*Kernel 2 End*/ 
<@\color{white}{.}@> 
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{.59\textwidth}
\begin{lstlisting}[caption=Kernel with large data,frame=tlrb]{}
<@\color{mauve}{float func(struct object x) \{ }@> 
<@\color{mauve}{	return ...; }@> 
<@\color{mauve}{\}}@> 
void func2(int N, struct object B[N]) {
	...
	// Kernel with data larger than the GPU memory can support
	<@\color{blue}{for(int i=0; i<N; i++) \{}@> 
		<@\color{blue}{A[i] = func(B[i]);}@> 
	<@\color{blue}{\}}@> 
}
\end{lstlisting}
\end{minipage}\vspace{-1.5em}
\noindent
\begin{minipage}{.39\textwidth}
\begin{lstlisting}[caption=Code generated from Code 1 to fuse two kernels reusing data and moving some serial code out of kernel,frame=tlrb]{Name}
<@\color{red}{\#pragma omp target teams map(A)}@>
<@\color{red}{\{}@> 
//Kernels fused together
/*Parallel Loop 1 using array A*/
<@\color{red}{\#pragma omp distribute parallel for}@>
for(...) { ... }
/*Parallel Loop 2 using array A*/
<@\color{red}{\#pragma omp distribute parallel for}@>
for(...) { ... }
<@\color{red}{\}}@>
<@\color{mauve}{/*Serial Code Start }@>
<@\color{mauve}{...}@>  <@\color{dkgreen}{// Moved out of the kernels}@>
<@\color{mauve}{Serial Code End*/}@>
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{.59\textwidth}
\begin{lstlisting}[caption=Code Generated from Code 2 for decomposing a large kernel and splitting the computation over multiple devices,frame=tlrb]{Name}
<@\color{red}{\#pragma omp declare target}@>
<@\color{mauve}{float func(struct object x) \{ return ...; \}}@>
<@\color{red}{\#pragma omp end declare target}@>
void func2(int N, struct object B[N]) {
	...
	//Decomposing Kernel and splitting computation over two GPUs
	<@\color{red}{\#pragma omp target enter data map(alloc:A[0:N/2]) map(to:B[0:N/2]) device(0)}@>
	<@\color{red}{\#pragma omp target teams distribute parallel for device(0)}@>
	<@\color{blue}{for(int i=0; i<N/2; i++) \{ A[i] = func(B[i]); \}}@>
	<@\color{dkred}{\#pragma omp target enter data map(alloc:A[N/2:N/2]) map(to:B[N/2:N/2]) device(1)}@>
	<@\color{dkred}{\#pragma omp target teams distribute parallel for device(1)}@>
	<@\color{blue}{for(int i=N/2; i<N; i++) \{ A[i] = func(B[i]); \}}@>
}
\end{lstlisting}
\end{minipage}\vspace{-1.5em}
\caption{Samples of code generated for fusing and/or decomposing kernels}
\label{fig:code}
\end{figure*}

==> text/result.tex <==
\input{fig/plot_data_time}
\section{Results}
\label{sec:results}

For the first experiment on Data Analysis, we found that the Advisor improved the data management in all cases.
Figure~\ref{plot:data} shows the amount of data transferred (in GB) between the CPU and the GPU before and after transformation for all benchmark applications.
After applying our transformation, we can clearly see that the amount of data transfer has indeed been considerably reduced.
Reduced data transfer has an impact on all applications' data transfer times.
On all the available clusters, we ran these applications and collected the data transfer times.
Figure~\ref{plot:transfertime} shows the data transfer time for the Wilson Dslash Operator across different clusters.

In the second experiment on code generation, we count the number of kernels identified and the number of codes generated for each application.
Table~\ref{tab:advisor:result:codegen} shows the result of this experiment.
We compiled all of these codes for various clusters using the compilers shown in Table~\ref{tab:advisor:cluster}.
Some compilers (NVIDIA/nvc) do not support dynamic or guided scheduling on a GPU, resulting in compilation failure.
Apart from that, all of the codes successfully compiled and ran on their respective clusters.
We collected the runtime of each of the kernels in this experiment.

\input{table/result_codegen}

The Cost Model is put to the test in the third experiment.
Cost model functions differently in the Training mode and the Prediction mode.
In the training mode, we train our cost model using all of the data from the previous experiment.
We can see that a simple MLP performs admirably in all of our applications, as evidenced by the strong correlation between actual and predicted data in Figure~\ref{fig:validate}.
Seawulf has NVIDIA K80 GPUs, which is the slowest of the GPUs we're using in our experiment.
So each kernel runs longer on Seawulf than it would on any other cluster.
Due to this, compared to other clusters, very little data (for larger kernel) was collected on Seawulf.
As a result, for larger data sets, the model trained for Seawulf does not perform very well.

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{fig/validation.png}
	\caption{Validation of Cost Model on different clusters}
	\label{plot:validate}
\end{figure}

Finally we used our Advisor to predict for Wilson Dslash kernel.

\input{fig/plot_prediction}
\input{fig/plot_prediction_rmse}

